NerfAcc: Efficient Sampling Accelerates NeRFs

Optimizing and rendering Neural Radiance Fields is computationally expensive due to the vast number of samples required by volume rendering. Recent works have included alternative sampling approaches to help accelerate their methods, however, they are often not the focus of the work. In this paper, we investigate and compare multiple sampling approaches and demonstrate that improved sampling is generally applicable across NeRF variants under an unified concept of transmittance estimator. To facilitate future experiments, we develop NerfAcc, a Python toolbox that provides flexible APIs for incorporating advanced sampling methods into NeRF related methods. We demonstrate its flexibility by showing that it can reduce the training time of several recent NeRF methods by 1.5x to 20x with minimal modifications to the existing codebase. Additionally, highly customized NeRFs, such as Instant-NGP, can be implemented in native PyTorch using NerfAcc.

==> figures/ray_marching.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=\linewidth]{figures/assets/ray_marching.pdf}
\caption{\textbf{Different Efficient Ray Marching Approaches} \textit{(a) Proposal Net}: A network (or more) is trained with SGD to build the PDF of the surface location along the ray. Multiple rounds of radiance field query are require during both training and inference. (b) \textit{(a) Occ Grid}: An explicit voxel grid is updated during training to keep track of the \textit{maximum} occupancy at each cell for skipping or pruning. The voxel grid is updated with extra radiance field query during training. (c) \textit{Proposal Grid}: An explicit voxel grid is updated during training to keep track of the \textit{average} occupancy of space, where the PDF is build from. The density grid is be updated with training samples.
}
\label{fig:ray_marching}
\end{figure*}

==> tables/volrend_psnr.tex <==

\begin{table}[t]
    \centering
    \tablestyle{2pt}{1.05}
    \begin{tabular}{lcccc}
        \toprule
        {} & 
        PSNR~$\uparrow$ & 
        LPIPS~$\uparrow$ & 
        Time (sec)~$\downarrow$ &
        FPS ~$\uparrow$
        \\
        \midrule
        Occ Grid & 
        \textbf{32.55} & 
        \textbf{0.056} &
        \textbf{263} &
        3.12
        \\
        Proposal Grid & 
        31.94 & 
        0.059 &
        278 &
        \textbf{3.20}
        \\
        Proposal Net & 
        31.40 & 
        0.064 &
        310 &
        2.96
        \\
        \bottomrule
    \end{tabular}
    \vspace{0.5em}
    \caption{Different Ray Marching Approaches on \textit{NeRF-Synthetic} Dataset}
    \label{tab:volrend_syn}
\end{table}



\begin{table}[t]
    \centering
    \tablestyle{2pt}{1.05}
    \begin{tabular}{lcccc}
        \toprule
        {} & 
        PSNR~$\uparrow$ & 
        LPIPS~$\uparrow$ & 
        Time (sec)~$\downarrow$ &
        FPS ~$\uparrow$
        \\
        \midrule
        Occ Grid & 
        26.38 & 
        0.351 &
        330 &
        1.44
        \\
        Proposal Grid & 
        26.85 & 
        0.327 &
        315 &
        \textbf{2.20}
        \\
        Proposal Net & 
        \textbf{27.21} & 
        \textbf{0.300} &
        \textbf{299} &
        1.33
        \\
        \bottomrule
    \end{tabular}
    \vspace{0.5em}
    \caption{Different Ray Marching Approaches on the \textit{Mip-NeRF 360} Dataset}
    \label{tab:volrend_360}
\end{table}

